The Relevance of Muon Deflections for Neutrino Telescopes

Large-scale neutrino telescopes have the primary objective to detect and characterize neutrino sources in the universe. These experiments rely on the detection of charged leptons produced in the interaction of neutrinos with nuclei. Angular resolutions are estimated to be better than 1 degree, which is achieved by the reconstruction of muons. This angular resolution is a measure of the accuracy with which the direction of incoming neutrinos can be determined. Since muons can traverse distances of several kilometers through media, the original muon direction can differ from the muon direction inside the detector due to deflections by stochastic interactions and multiple scattering. In this contribution, a recently published study of muon deflections based on the simulation tool PROPOSAL is presented. Muons with various energies are propagated through different media over several distances. Data-Monte-Carlo comparisons as well as comparisons to the simulation tools MUSIC and Geant4 are performed. Finally, the impact of muon deflections on large-scale neutrino telescopes is discussed.

==> Makefile <==
all: build/skeleton.pdf

TeXOptions = -lualatex \
	-interaction=nonstopmode \
	-halt-on-error \
	-output-directory=build

build/skeleton.pdf: FORCE | build
	latexmk $(TeXOptions) skeleton.tex 

FORCE:

build:
	mkdir -p build 

clean: 
	rm -rf build

